A Competence-aware Curriculum for Visual Concepts Learning via Question Answering

Humans can progressively learn visual concepts from easy to hard questions. To mimic this efficient learning ability, we propose a competence-aware curriculum for visual concept learning in a question-answering manner. Specifically, we design a neural-symbolic concept learner for learning the visual concepts and a multi-dimensional Item Response Theory (mIRT) model for guiding the learning process with an adaptive curriculum. The mIRT effectively estimates the concept difficulty and the model competence at each learning step from accumulated model responses. The estimated concept difficulty and model competence are further utilized to select the most profitable training samples. Experimental results on CLEVR show that with a competence-aware curriculum, the proposed method achieves state-of-the-art performances with superior data efficiency and convergence speed. Specifically, the proposed model only uses 40% of training data and converges three times faster compared with other state-of-the-art methods.

==> rebuttal.tex <==
\clearpage
\section{Rebuttal}
\subsection{Reviewer 3}
We thank the reviewer for acknowledging the novelty of our ideas and the great performance of the experimental results. We respond to each question separately in the following.

Q1. "Which questions are being picked up over time?"

A1: Please refer to Fig.3 in the supplementary materials for exemplary questions selected at different training iterations. We observe that our model selects increasingly complex questions during the training progress. The training process starts with simple questions containing one or two concepts and moves to complex ones involving combined concepts with spatial relationships.

Q2. "Expect over time results of Fig.4."

A2: Thanks for the suggestion. We will add such a figure in our revision. Also, please note that we do have analyses on the model performance over time. For example, Fig.5 summarizes the model competence at various iterations for different attributes, Fig.2 in the supplementary materials also shows the accuracy of each concept at different iterations.

Q3. "It is a bit counterintuitive for the reader that colors are the hardest concepts." 

A3: It was a bit surprising for us as well. We guess it is largely due to the imbalanced number of concepts for each attribute in the CLEVR dataset. The CLEVR dataset has **8 colors**, but only 2 materials, 3 shapes, 2 sizes, and 4 spatial relations. Therefore, the model needs to learn a more sophisticated classifier to capture the subtle differences among 8 colors, making it hardest to learn.

Q4. "In Fig.3, it seems to indicate that the model at 0 iterations already has a decent accuracy in the training set."

A4: The accuracy on the training set is computed per batch, and our model selects a batch of simple questions containing only one or two concepts at the 0 iteration. These questions are easier to answer compared with randomly sampled questions, and our model achieves an accuracy of about 55\%, which is slightly higher than a random guess in binary classification.

Q5. "How is the object detector trained?"

A5: The object detector (Mask R-CNN) is pre-trained on 4k generated CLEVR images with bounding box annotations only. We use ResNet-50 FPN as the backbone and train the model for 30k iterations with a batch size of 8. Please refer to Sec.1 in the supplementary materials for more training details.

Q6. "The tables with results are very hard to read."

A6: We will make the numbers in tables (especially Tab.3) larger in our revision.

\clearpage
\subsection{Reviewer 1}
We thank the reviewer for acknowledging our work is refresh and sound and respond to the questions below:

>Q1. Comparison with uncertainty sampling.

We tried uncertainty sampling but found it infeasible in our scenario. Specifically, uncertainty sampling requires to evaluate the model on all the 700k questions in the training set to calculate the output probability and uncertainty, which takes more than five hours using an Nvidia Titan Xp GPU. This evaluation process needs to be repeated every time we select a new subset for training. Therefore, directly using uncertainty sampling is too time-consuming to be practical in our case. We believe this is the main drawback of traditional active learning methods since they are designed to deal with a small amount of data. In contrast, our model uses accumulated responses to avoid time-consuming evaluation. We guess a better approach might combine the mIRT and uncertainty sampling: first, use mIRT to select a subset of questions from the whole training set, and then perform uncertainty sampling over this subset. We leave this possibility for future work.

>Q2. In Fig. 3, NSCL-mIRT has higher accuracy than other methods with 0 training data.

Please refer to Q4 for Reviewer 3.

>Q3. The x-axis in Fig. 3 isn't the number of samples used.

Yes, the samples are cycled throughout iterations and used multiple times. The "number of samples" in Fig.3 denotes "number of iterations * batch size," which is larger than "unique questions" in Line 492. For example, when NSCL-mIRT converges with ~800k training samples in Fig.3, we find there are ~300k unique samples and each sample is repeatedly used for 2.6 times on average. We will make the conclusion more clear in our revision.

>Q4. NSCL doesn't improve over the first 700k iterations.

We empirically observe this "cold start" problem for NSCL without any curriculum, which is the same observation as [41]. The potential reason is that the model only has one pass of the CLEVR training set for the first 700k iterations, and the complex long questions could confuse the model at the first pass. Concept learning from question-answer pairs is similar to learning to align visual patterns with textual words, and complex questions involving too many concepts might hinder the learning process at the early stage.

>Q5. The drops in Fig.5 (a).

We suspect there are not sufficient model responses at the early stage, leading to an unstable estimation of mIRT using variational inference.

%>Q6. What is g in Eq.6?

%As stated in Line 352, g\_j is the probability of guessing the correct answer to the j-th question.



%A2: The accuracy on the training set is computed per batch, and our model selects a batch of simple questions containing only one or two concepts at the 0 iteration. These questions are easier to answers after training, and our model achieves an accuracy of about 55\%, which is reasonable since it is slightly higher than a random guess in binary classification. {\color{red}The other methods randomly sample questions from the training set or learn from a manually-designed discretized curriculum, which makes the learning harder and the training accuracy lower at the beginning. (Why the manually-designed is almost the same with randomly sample?)}

\clearpage
\subsection{Reviewer 2}
We thank the reviewer for valuable comments and respond to the major concerns in the following. Minor issues will be addressed in the revision and not be discussed here due to the space limit. 

>[W0] Missing a simple baseline.

A: Please refer to Q1 for Reviewer 1. 

>[W1] Why is c\_j replaced by g\_j in eq. 6?

A: There are two reasons for using guessing parameter at question level: (1) NSCL performs reasoning in a probabilistic manner with concept recognition results, i.e., no guessing is made in the concept level and all possibilities are kept during the reasoning process, guessing only happens when the model generates the final answer, depending on the question type; (2) in the literature of IRT, the guessing parameter is usually set at the response level, i.e., the question level in our case since we only have responses on the question level, not on the concept recognition level.

>[W1] The scale factor a\_j disappears.

A: We tried to use a\_j, but it empirically made no differences. Actually, in the practices of IRT, the scale factor is often abandoned as well. Therefore, we eliminate this parameter for simplicity.

>[W1] Limitations about Eq.6.

A: Good catch. It is a limitation of our current formulation. A possible remedy is to add a smoothing factor in Eq. 6 to avoid reverting to the guessing probability due to failing at a single concept.

>[W2] Setting Upper / Lower Bound Parameters.

A: We agree with your comments. Proper upper/lower bounds will roughly separate the learning process into four stages. First, LB takes effect by eliminating hard questions and UB has no influence. Second, both LB and UB take effect by filtering out too hard/easy questions. Third, the model's competence is high enough so that LB has no influence anymore and UB eliminates most simple questions. Finally, the model performs well across the whole training set and all questions are filtered out by UB, this triggers an early stopping of the training, as also shown in Fig.3, NSCL-mIRT stops at ~800k training samples. In our work, LB and UB are set as hyperparameters and tuned by cross-validation. We look forward to developing an automatic method to tune these two parameters in the future.

>[W3] More analysis.

A: Please refer to Fig.3 in the supplementary materials for exemplary questions selected at different training iterations. By comparing the ids of selected questions, we find that the generated curriculum is fairly consistent across different runs.

%[Minor issues] What is the Mark R-CNN pretrained on? \\
%A:  Please refer to Q5 for Reviewer 3.


%We tried this simple approach, but found it infeasible due to the inefficiency. To select a "just difficult enough" subset at iteration j, it requires evaluating the current model on every question in the whole training set to compute the model's output probability of the correct answer. After training for a certain time, we need to repeat this process to select a new subset for the updated model. {\color{red}Do we need to add some numbers here}. This procedure is too time-consuming to be practical. In contrast, the mIRT model uses the accumulated model responses (at no cost since we already have them during training) to estimate the concept difficulty and model competence, and then select proper questions (the additional time cost is negligible as stated in Line 488).

%---The pre-equation exploration starting at L348 is difficult to work through. \\
%A: We will revise this part accordingly and make it easier to understand incrementally.
